A Scalable Algorithm for Shape Optimization with Geometric Constraints in Banach Spaces

This work develops an algorithm for PDE-constrained shape optimization based on Lipschitz transformations. Building on previous work in this field, the $p$-Laplace operator is utilized to approximate a descent method for Lipschitz shapes. In particular, it is shown how geometric constraints are algorithmically incorporated avoiding penalty terms by assigning them to the subproblem of finding a suitable descent direction. A special focus is placed on the scalability of the proposed methods for large scale parallel computers via the application of multigrid solvers. The preservation of mesh quality under large deformations, where shape singularities have to be smoothed or generated within the optimization process, is also discussed. It is shown that the interaction of hierarchically refined grids and shape optimization can be realized by the choice of appropriate descent directions. The performance of the proposed methods is demonstrated for energy dissipation minimization in fluid dynamics applications.

==> notes.tex <==
\section{Notes}

\todo{This section is just for us to make some notes and shall not be included within the final draft.}

\subsection{Schur GMRES}

\begin{algorithm}
\caption{GMRES for Schur Complement with $2$-times Gram-Schmidt}
\begin{algorithmic}
    \Require{$A \in \mathbb{R}^{n\times n}$, $B \in \mathbb{R}^{n \times (d+1)}$, $f \in \mathbb{R}^n$, $g \in \mathbb{R}^{d+1}$, $m \in \mathbb{N}$, $\epsilon > 0$, $y_0 \in \mathbb{R}^{d+1}$}
    \State{$w \gets A^{-1} f$} \Comment{e.g. GMRES or CG}
    \State{$b \gets g - B^T w$}
    \State{$u \gets B y$}
    \State{$v \gets A^{-1} u$}
    \State{$r \gets b + B^T v$}
    \State{$\beta_1 \gets \| r \|_2$}
    \State{$q_1 \gets r / \beta_1$}
    \For{$j = 1, \ldots m$}
        \State{\color{orange}$u \gets B q_j$}
        \State{\color{orange}$v \gets A^{-1} u$} \Comment{e.g. GMRES or CG}
        \State{\color{orange}$r \gets B^T v$}
        \For{$i = 1, 2$}
            \State{$c_k \gets q_k^T r$ for $k = 1, \ldots, j$}
            \State{$r \gets r - \sum_{k = 1}^j q_k c_k$}
            \State{$h_{k,j+1} \gets h_{k,j+1} + c_k$ for $k = 1, \ldots, j$}
        \EndFor
        \State{$h_{j+1,j} \gets \| r \|_2$}
        \State{$q_{j+1} \gets r / h_{j+1,j}$}
        %
        \For{$i = 1, \ldots, j-1$}
            \State{$t \gets c_i h_{i,j} + s_i h_{i+1,j}$}
            \State{$h_{i+1,j} \gets - s_i h_{i,j} + c_i h_{i+1,j}$}
            \State{$h_{i,j} \gets t$}
        \EndFor
        \State{$[c_j, s_j] \gets \textsc{givens}(h_{j,j}, h_{j+1,j})$}
        %
        \State{$\beta_{j+1} \gets - s_j \beta_j$}
        \State{$\beta_{j} \gets c_j \beta_j$}
        %
        \If{$\beta_{j+1} \leq \tau \| b \|$}
            \State break
        \EndIf
    \EndFor
    %
    \For{$i = j, \ldots, 1$}
        \State{$z_i \gets \left( \beta_i - \sum_{k = i+1}^j h_{i,k} z_k \right) / h_{i,i}$} \Comment{back substitution}
    \EndFor
    \State{$y \gets y_0 + \sum_{i = 1}^j q_i z_i$}
    \State{$x \gets A^{-1}(f - B y)$} \Comment{soving for $x$ e.g. GMRES or CG}
\end{algorithmic}
\end{algorithm}

\begin{lstlisting}[language=Octave]
function [x, y, iter, res] = mySchurGMRES(A, b1, b2, b3, b4, 
  f, g, x, y, maxIter, tol)
    
  n = 4;
  na = size(A)(1);
  
  m = maxIter;
  reltol = tol * norm(g);

  % Start Schur-GMRES
  Q = zeros(n,m+1);
  H = zeros(m+1,m);
  beta = zeros(m+1,1);
  cs = zeros(m,1);
  sn = zeros(m,1);
  c = zeros(n,1);
  w = zeros(na,1);
  v = zeros(na,1);

  % Determine right hand side
  [w, iter1, res1] = myGMRES(A, f, w, na, tol);
  %b = g - B' * w;
  b = zeros(n,1);
  b(1) = g(1) - dot(b1, w);
  b(2) = g(2) - dot(b2, w);
  b(3) = g(3) - dot(b3, w);
  b(4) = g(4) - dot(b4, w);

  % Compute initial residual
  %u = B * y;
  u = zeros(na,1);
  for i = 1:na
    u(i) = b1(i) * y(1) + b2(i) * y(2) + b3(i) * y(3)...
           + b4(i) * y(4);
  endfor

  %v = A \ u;
  [v, iter1, res1] = myGMRES(A, u, v, na, tol);
  %r = b + B' * v;
  r = zeros(n,1);
  r(1) = b(1) + dot(b1, v);
  r(2) = b(2) + dot(b2, v);
  r(3) = b(3) + dot(b3, v);
  r(4) = b(4) + dot(b4, v);

  
  beta(1) = norm(r);
  Q(:,1) = r / beta(1);
  res = abs(beta(1));

  
  for j = 1:m
    
    % Arnoldi
    %u = B * Q(:,j);
    for i = 1:na
      u(i) = b1(i) * Q(1,j) + b2(i) * Q(2,j) + b3(i) * Q(3,j) ...
             + b4(i) * Q(4,j);
    endfor
    %v = A \ u;
    v = zeros(na,1);
    [v, iter, res] = myGMRES(A, u, v, na, tol);
%    r = - B' * v;
     r(1) = -dot(b1, v);
     r(2) = -dot(b2, v);
     r(3) = -dot(b3, v);
     r(4) = -dot(b4, v);
    
    for i = 1:2
      c = Q(:,1:j)'*r;
      r = r - Q(:,1:j)*c;
      H(1:j,j) = H(1:j,j) + c;
    endfor

    H(j+1,j) = norm(r);
    Q(:,j+1) = r / H(j+1,j);
    
    % Givens
    for i = 1:j-1
      tmp = cs(i) * H(i,j) + sn(i) * H(i+1,j);
      H(i+1,j) = -sn(i) * H(i,j) + cs(i) * H(i+1,j);
      H(i,j) = tmp;
    endfor  
    [H(j:j+1,j), cs(j), sn(j)] = gvn(H(j:j+1,j));

    beta(j+1) = -sn(j) * beta(j);
    beta(j) = cs(j) * beta(j);
    res = abs(beta(j+1));
    
    if res <= reltol;
      break;
    endif
  endfor
  iter = j;
 
  z = zeros(j,1);
  for i = j:-1:1
    z(i) = (beta(i) - dot(H(i,i:j),z(i:j))) / H(i,i);
  endfor

  y = y +  Q(:,1:j)*z;
 
  % u = f - B * y;
  for i = 1:na
    u(i) = f(i) - b1(i) * y(1) - b2(i) * y(2) - b3(i) * y(3)...
           - b4(i) * y(4);
  endfor
  [x, iter2, res2] = myGMRES(A, u, x, na, tol);
    
endfunction
\end{lstlisting}


\subsection{Discretization}

Discretization of the column within the matrix $B$ and row within $B^T$, respectively, corresponding to the volume constraint.


\begin{equation}
    w(x) \approx w_h(x) = \sum_{i = 1}^n \phi_i(x) w_{i}, \qquad w_i = w (x_i)
\end{equation}

\begin{equation}
    \nabla w_j(x) \approx \nabla w_{hj}(x) = \sum_{i = 1}^n \nabla \phi_i(x) w_{ji}, \qquad w_{ji} = w_j(x_i)
\end{equation}
%
where $w_j(x)$ is the $j$-th component of the vector $w(x)$.
%
\begin{equation}
    Dw = 
    \begin{pmatrix}
    \nabla w_1(x)^T \\
    \vdots \\
    \nabla w_d(x)^T
    \end{pmatrix}
\end{equation}
%
$DF^{-1} \coloneqq (a_{ij})_{i,j = 1, \ldots,d}$, $Dw \coloneqq (c_{ij})_{i,j = 1, \ldots, d}$
%
\begin{equation*}
    DF^{-1} Dw = \left( \sum_{k = 1}^d a_{ik} c_{kj} \right)_{i,j = 1, \ldots, d}
\end{equation*}
%
\begin{equation*}
    tr(DF^{-1} Dw) = \sum_{l = 1}^d \left( \sum_{k = 1}^d a_{lk} c_{kl} \right) 
\end{equation*}
%
$c_{kl} = \frac{\partial w_k}{\partial x_l} \approx \sum_{i = 1}^n \frac{\partial \phi_i}{\partial x_l}(x) w_{ki}$
%
\begin{gather*}
    tr(DF^{-1} Dw) \approx \sum_{l = 1}^d \sum_{k = 1}^d a_{lk} \left( \sum_{i = 1}^n \frac{\partial \phi_i}{x_l}(\partial x) w_{ki} \right) 
    = \sum_{i = 1}^n \left( \sum_{l = 1}^d \sum_{k = 1}^d a_{lk} \frac{\partial \phi_i}{\partial x_l}(x) w_{ki} \right) \\
    = \sum_{i = 1}^n \nabla \phi_i^T(x) DF^{-1}(x) w_i
\end{gather*}


\begin{equation}
    \int_\Omega 
        tr(DF^{-1} Dw) \det{DF} 
    \; dx \approx 
    \sum_{i = 1}^d 
    \underbrace{\int_\Omega 
        \nabla \phi_i(x) DF^{-1} \det{DF}
    \; dx}_{\let\scriptstyle\textstyle\substack{\text{row vector} \; (b_{1i}, \ldots, b_{di})}} \, w_i
\end{equation}

\subsection{Step size control}

With $F = \id + u$ the functional to be minimized 
\begin{gather}
    L(u,\lambda) := \frac{1}{p} \int_\Omega (\nabla u : \nabla u)^{p/2} \; dx 
    + J^\prime(\Omega; u) \nonumber \\
    + \sum_{i=1}^d \lambda_i \int_\Omega (x_i + u_i) \det(DF) \; dx 
    + \lambda_{d+1} \int_\Omega \det(DF) \; dx
\end{gather}
Now with a step size $t > 0$ the descent direction may be written as $u := tv \in W^{1,p}$ and therewith
\begin{gather}
    L(tv,\lambda) := \frac{1}{p} \int_\Omega \left(\nabla (tv) : \nabla (tv) \right)^{p/2} \; dx 
    + J^\prime(\Omega; tv) \nonumber \\
    + \sum_{i=1}^d \lambda_i \int_\Omega (x_i + tv_i) \det(DF_t) \; dx 
    + \lambda_{d+1} \int_\Omega \det(DF_t) \; dx
\end{gather}
where $F_t = \id + tv$. Obviously 
\begin{equation}
    \left(\nabla (tv) : \nabla (tv) \right)^{p/2} = \left(t^2 \nabla v : \nabla ) \right)^{p/2} = t^p \left(\nabla v : \nabla v \right)^{p/2}
\end{equation}
holds and because $J^\prime$ is linear regarding $u$ and $tv$, respectively,
\begin{equation}
    J^\prime(\Omega; tv) = t J^\prime(\Omega; v)
\end{equation}
holds. Exemplary for the case $d = 3$ the determinant of the jacobian of $F_t$ reads 
\begin{gather*}
    \det(DF_t) = t^{3} \left(v_{11} v_{22} v_{33} - v_{11} v_{23} v_{32} - v_{12} v_{21} v_{33}
    + v_{12} v_{23} v_{31} + v_{13} v_{21} v_{32} - v_{13} v_{22} v_{31}\right) \\
    + t^{2} \left(v_{11} v_{22} + v_{11} v_{33} - v_{12} v_{21} - v_{13} v_{31} + v_{22} v_{33} - v_{23} v_{32}\right) \\ 
    + t \left(v_{11} + v_{22} + v_{33}\right) \\
    + 1
\end{gather*}
or in a more easy to read way 
\begin{equation*}
    \det(DF_t) = \sum_{k = 0}^3 t^k f_k(\nabla v).
\end{equation*}
Inserting this into the Functional one can see how the terms scale with the step size $t>0$:
\begin{gather*}
    L(tv,\lambda) := \underbrace{\frac{t^p}{p} \int_\Omega (\nabla tv : \nabla tv)^{p/2} \; dx}_{\propto t^p} 
    + \underbrace{t J'(\Omega; v)}_{\propto t} \nonumber \\
    + \underbrace{\sum_{i=1}^d \lambda_i \int_\Omega (x_i + tv_i) \sum_{k = 0}^3 t^k f_k(\nabla v) \; dx}_{\propto t^4}
    + \underbrace{\lambda_{d+1} \int_\Omega \sum_{k = 0}^3 t^k f_k(\nabla v) \; dx}_{\propto t^3}
\end{gather*}


\begin{gather}
    L(u,\lambda) := \frac{1}{p} \int_\Omega (\nabla u : \nabla u)^{p/2} \; dx 
    + t^{p-1} J^\prime(\Omega; u) \nonumber \\
    + \sum_{i=1}^d \lambda_i \int_\Omega (x_i + u_i) \det(DF) \; dx 
    + \lambda_{d+1} \int_\Omega \det(DF) \; dx
\end{gather}
